An Efficient Summation Algorithm for the Accuracy, Convergence and Reproducibility of Parallel Numerical Methods

Nowadays, parallel computing is ubiquitous in several application fields, both in engineering and science. The computations rely on the floating-point arithmetic specified by the IEEE754 Standard. In this context, an elementary brick of computation, used everywhere, is the sum of a sequence of numbers. This sum is subject to many numerical errors in floating-point arithmetic. To alleviate this issue, we have introduced a new parallel algorithm for summing a sequence of floating-point numbers. This algorithm which scales up easily with the number of processors, adds numbers of the same exponents first. In this article, our main contribution is an extensive analysis of its efficiency with respect to several properties: accuracy, convergence and reproducibility. In order to show the usefulness of our algorithm, we have chosen a set of representative numerical methods which are Simpson, Jacobi, LU factorization and the Iterated power method.

==> background.tex <==

Following the IEEE754 Standard, a floating-point number $x$ in base $\beta$ is given by Equation~(\ref{flottants}).
\begin{equation}
x=s \cdot (d_{0}\cdot d_{1}\cdot d_{f-1})\cdot\beta^{exp}=s\cdot m\beta^{exp-f+1}
\label{flottants}
\end{equation}
where
\begin{itemize}
\item $s \in \{-1,1\}$ is the sign,
\item $m=d_{0}d_{1}....d_{f-1}$ is the mantissa with digits $0\leq d_{i} <\beta$, $0\leq i\leq f-1$,
\item $f$ is the precision,
\item $exp$ is the exponent with $exp_{min}\leq exp\leq exp_{max}$.
\end{itemize}
The IEEE754 Standard defines binary formats with some particular values for $f$, $exp_{min}$ and $exp_{max}$ which are summarized in Table~\ref{formats}. 
Moreover, the IEEE754 Standard defines four rounding modes for elementary operations over floating-point numbers. These modes are towards $+\infty$ ,towards $-\infty$, towards zero and towards nearest denoted by $\circ_{+\infty}$, $\circ_{-\infty}$, $\circ_{0}$ and $\circ_{\sim}$, respectively.
%For $\mathbb{R}$ a set of real numbers and $\mathbb{F}$ a set of floating-point numbers.
%Let $\uparrow_{\circ}:\mathbb{R}\to\mathbb{F}$ be the function which returns the roundoff of a real number following the rounding mode $\circ\in\{\circ_{+\infty}, \circ_{-\infty}, \circ_{0},\circ_{\sim}\}$.
The behavior of the elementary operations $\diamond\in\{+,-,\times,\div\}$ between floating-point numbers is given by Equation~\ref{error} 
\begin{equation}\label{error}
v_1\diamond_{\circ}v_2=\circ(v_1\diamond v_2)
\end{equation}
where $\circ$ denotes the rounding mode such as $\circ\in\{\circ_{+\infty}, \circ_{-\infty}, \circ_{0},\circ_{\sim}\}$.
By Equation~\ref{error}, we illustrate that in floating-point computations, performing an elementary operation $\diamond_\circ$ with rounding mode $\circ$ returns the same result to the one obtained by an exact operation $\diamond$, then rounding the result using $\circ$.
The IEEE754 Standard also specifies how the square root function must be rounded 
in a similar way to Equation~\ref{error} but does not specify the roundoff of other functions like sin, log, etc.
\begin{table}[t]
\centering
\begin{tabular}{|cccccc|}
\hline
Format               & \hspace{0.3cm} $\#$total bits & \hspace{0.3cm}$f$ bits & \hspace{0.3cm}$exp$ bits & \hspace{0.3cm}$exp_{min}$ & \hspace{0.3cm}$exp_{max}$\\
\hline
Half precision       & \hspace{0.3cm}$16$ bits      &\hspace{0.3cm} $11$      & \hspace{0.3cm}$5$       & \hspace{0.3cm}$-14$    &\hspace{0.3cm} $+15$ \\
Single precision     & \hspace{0.3cm}$32$ bits      &\hspace{0.3cm} $24$      & \hspace{0.3cm}$8$       & \hspace{0.3cm}$-126$   & \hspace{0.3cm}$+127$ \\
Double precision     & \hspace{0.3cm}$64$ bits      &\hspace{0.3cm} $53$      & \hspace{0.3cm}$11$      & \hspace{0.3cm}$-1122$  & \hspace{0.3cm}$+1223$\\
Quadruple precision  & \hspace{0.3cm}$128$ bits     &\hspace{0.3cm}$113$      & \hspace{0.3cm}$15$      & \hspace{0.3cm}$-16382$ &\hspace{0.3cm}$+16383$ \\
\hline
\end{tabular}
\caption{Binary formats of IEEE754 Standard\label{formats}} 
\end{table}
In this article, without loss of generality, we consider that $\beta=2$. 
Moreover, we assume that no overflow occurs and we only consider the rounding mode to the nearest.
In floating-point computations absorption and cancellation may affect the numerical accuracy of computations.
An absorption occurs when adding two floating-point numbers with different orders of magnitude. The small value is absorbed by the large one.
For example, when computing the sum $s=((x+y)+z)$ such that $x$, $y$ and $z$ 
are three floating-point numbers stored in binary 32 format, where $x =1.2\times 2^{0} $ , $y=1\times 2^{24}$ and $z=-1\times 2^{24}$, respectively. 
Then, the computation of $s$ produces the result $s=0.0$ which has no correct digits, 
as the correct real result should be $s=1.2\times 2^{0}$.\\
A cancellation occurs when two nearly equal numbers are subtracted and the most significant digits cancel each other. 
The severity of the cancellation differs from one computation to another depending on the number of useful bits lost.
For example, let $x=1.5\times 2^{0}$ and $y=1\times 2^{24}$ two floating-point numbers in single precision. The computation of the sequence of operations $s=((x+y)-y)$ 
produces the result $s=0.0$ while the real result should be $1.5\times 2^{0}$.


hhhh

